GD^2-NeRF: Generative Detail Compensation via GAN and Diffusion for One-shot Generalizable Neural Radiance Fields

In this paper, we focus on the One-shot Novel View Synthesis (O-NVS) task which targets synthesizing photo-realistic novel views given only one reference image per scene. Previous One-shot Generalizable Neural Radiance Fields (OG-NeRF) methods solve this task in an inference-time finetuning-free manner, yet suffer the blurry issue due to the encoder-only architecture that highly relies on the limited reference image. On the other hand, recent diffusion-based image-to-3d methods show vivid plausible results via distilling pre-trained 2D diffusion models into a 3D representation, yet require tedious per-scene optimization. Targeting these issues, we propose the GD$^2$-NeRF, a Generative Detail compensation framework via GAN and Diffusion that is both inference-time finetuning-free and with vivid plausible details. In detail, following a coarse-to-fine strategy, GD$^2$-NeRF is mainly composed of a One-stage Parallel Pipeline (OPP) and a 3D-consistent Detail Enhancer (Diff3DE). At the coarse stage, OPP first efficiently inserts the GAN model into the existing OG-NeRF pipeline for primarily relieving the blurry issue with in-distribution priors captured from the training dataset, achieving a good balance between sharpness (LPIPS, FID) and fidelity (PSNR, SSIM). Then, at the fine stage, Diff3DE further leverages the pre-trained image diffusion models to complement rich out-distribution details while maintaining decent 3D consistency. Extensive experiments on both the synthetic and real-world datasets show that GD$^2$-NeRF noticeably improves the details while without per-scene finetuning.

==> Table/DTU_SOTA.tex <==

\begin{table}[t]
 \footnotesize
 \caption{
     \textbf{Comparisons with the state-of-the-art methods on the DTU dataset~\cite{DTU_jensen2014large}.}}
     \vspace{-3mm}
    \label{tab:DTU_SOTA}
    % \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{8pt}
        \begin{tabular}{l|cccc}
        \rowcolor[gray]{.9}
        \hline
        Methods           & $\uparrow$ PSNR                & $\uparrow$ SSIM               & $\downarrow$ LPIPS      & $\downarrow$ FID \\ \hline \hline                         
        PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf}   & {16.12}                         & {0.545}                    & 0.451             &  223.34   \\
        \textbf{OPP (ours)} & \textbf{16.19}      & \textbf{0.556}     & \textbf{0.392} & \textbf{149.95} \\ 
        \hline
        \end{tabular}
    % }
\end{table}

==> Table/Fewshot_Extension.tex <==
\begin{table}[t!]
     \caption{\textbf{Effectiveness of our OPP under the few-shot setting.}}
     \label{tab:fewshot_extension}
     \vspace{-4mm}
  % \resizebox{\linewidth}{!}{
% \setlength{\columnwidth}{15mm}{
\setlength\tabcolsep{9pt}
   \begin{tabular}{c|lccc}
        \rowcolor[gray]{.9}
        \hline
        \multicolumn{1}{l|}{Shot}   & Methods & $\uparrow$ PSNR            & $\downarrow$ LPIPS          & $\downarrow$ FID             \\ \hline \hline
        \multirow{2}{*}{2} & PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf}     & 17.62          & 0.378          & 194.71          \\
                                & \textbf{OPP}   & \textbf{17.75} & \textbf{0.345} & \textbf{143.38} \\ \hline
        \multirow{2}{*}{3} & PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf}     & 18.30          & 0.358          & 182.67          \\
                                & \textbf{OPP}   & \textbf{18.45} & \textbf{0.323} & \textbf{134.24} \\ \hline
        \end{tabular}
    % }
\end{table}

==> Table/NMR_SOTA.tex <==

\begin{table*}[t]
\setlength{\abovecaptionskip}{0cm}
\footnotesize
    {\caption{\textbf{Comparisons with the state-of-the-art methods under the category-agnostic setting ($64 \times 64$ resolution).} The performance of our final One-stage Parallel Pipeline (OPP) is reported.  ``\dag'' means that a test-time optimization is required. We attain a new state-of-the-art performance with a single model trained across all 13 classes.} 
  \label{tab:category_agnostic}}
% \vspace{-3mm}
  \begin{adjustbox}{width=\linewidth,center}
      \begin{tabular}{l| l c c c c c c c c c c c c c c}
        \rowcolor[gray]{.9}
        \hline
        Metrics & Methods & plane & bench & cbnt. & car & chair & disp. & lamp & spkr. & rifle & sofa & table & phone & boat & average \\
         \hline \hline
        \multirow{5}{*}{$\uparrow$ PSNR}    & SRN~\cite{SRN_sitzmann2019scene}~\dag      & 26.62 & 22.20 & 23.42 & 24.40 & 21.85 & 19.07 & 22.17 & 21.04 & 24.95 & 23.65 & 22.45 & 20.87 & 25.86 & 23.28 \\
                                           & PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf} & 29.76 & 26.35 & 27.72 & 27.58 & 23.84 & 24.22 & 28.58 & 24.44 & 30.60 & 26.94 & 25.59 & 27.13 & 29.18 & 26.80\\
                                           & FE-NVS~\cite{FE_NVS_guo2022fast}    & 30.15 & 27.01 & 28.77 & 27.74 & 24.13 & 24.13 & 28.19 & 24.85 & 30.23 & 27.32 & 26.18 & 27.25 & 28.91 & 27.08 \\ 
                                           % & FWD       & 30.01 & 26.16 & 28.49 & 27.01 & 23.44 & 24.00 & 27.84 & 24.45 & {30.40} & 26.76 & 25.91 & {27.61} & 28.69 & 26.66 \\
                                           & {SRT}~\cite{srt22}       & {31.47} & {28.45} & \textbf{30.40} & {28.21} & {24.69} & {24.58} & {28.56} & {25.61} & 30.09 & {28.11} & {27.42} & {28.28} & {29.18} & {27.87} \\
                                        %   \cline{2-16}
                                       
                                        %  &\textbf{OPP-N}& \underline{31.05} & \underline{28.06} & {29.24} & \underline{28.52} & \underline{25.16} & {25.31} & {28.76} & {25.44} & \underline{31.44} & \underline{28.19} & {27.21} & {27.91} & \underline{30.06} & \underline{28.00} \\
                                        %  &\textbf{OPP-G}& {30.83} & {27.92} & \underline{29.33} & {28.17} & {25.10} & \underline{25.35} & \textbf{29.22} & \underline{25.49} & {31.11} & {28.05} & \underline{27.29} & \underline{28.06} & {29.76} & {27.90} \\
                                         &\textbf{OPP (ours)}& \textbf{31.64} & \textbf{28.52} & {30.00} & \textbf{28.92} & \textbf{25.55} & \textbf{25.61} & \textbf{29.46} & \textbf{25.92} & \textbf{31.80} & \textbf{28.56} & \textbf{27.81} & \textbf{28.48} & \textbf{30.28} & \textbf{28.47} \\
         \hline
        \multirow{5}{*}{$\uparrow$ SSIM}    & SRN~\cite{SRN_sitzmann2019scene}~\dag       & 0.901 & 0.837 & 0.831 & 0.897 & 0.814 & 0.744 & 0.801 & 0.779 & 0.913 & 0.851 & 0.828 & 0.811 & 0.898 & 0.849 \\
                                           & PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf} & 0.947 & 0.911 & 0.910 & 0.942 & 0.858 & 0.867 & 0.913 & 0.855 & 0.968 & 0.908 & 0.898 & 0.922 & 0.939 & 0.910 \\
                                           & FE-NVS~\cite{FE_NVS_guo2022fast}    & 0.957 & 0.930 & 0.925 & 0.948 & 0.877 & 0.871 & 0.916 & 0.869 & 0.970 & 0.920 & 0.914 & 0.926 & 0.941 & 0.920 \\
                                           % & FWD       & 0.952 & 0.914 & 0.918 & 0.939 & 0.857 & {0.867} & 0.906 & {0.857} & {0.968} & 0.909 & 0.906 & 
                                           % {0.924} & 0.936 & 0.911 \\
                                           & {SRT}~\cite{srt22}       & {0.954} & {0.925} & {0.920} & 0.937 & {0.861} & 0.855 & 0.904 & 0.854 & 0.962 & {0.911} & {0.909} & 0.918 & 0.930 & {0.912} \\
                                        % \cline{2-16}
                                        % &\textbf{OPP-N}& \underline{0.961} & \underline{0.937} & {0.926} & \underline{0.953} & {0.890} & \underline{0.886} & \underline{0.921} & {0.873} & {0.974} & \underline{0.926} & {0.924} & {0.929} & \underline{0.950} & {0.929} \\
                                        %  &\textbf{OPP-G}& {0.960} & {0.937} & \underline{0.928} & {0.951} & \underline{0.892} & \textbf{0.890} & \textbf{0.925} & \underline{0.877} & \underline{0.975} & \underline{0.926} & \underline{0.927} & \underline{0.932} & {0.949} & \underline{0.930} \\
                                         &\textbf{OPP (ours)}& \textbf{0.965} & \textbf{0.942} & \textbf{0.934} & \textbf{0.956} & \textbf{0.898} & \textbf{0.893} & \textbf{0.927} & \textbf{0.881} & \textbf{0.977} & \textbf{0.931} & \textbf{0.931} & \textbf{0.934} & \textbf{0.952} & \textbf{0.934} \\
         \hline
        \multirow{5}{*}{$\downarrow$ LPIPS} & SRN~\cite{SRN_sitzmann2019scene}~\dag       & 0.111 & 0.150 & 0.147 & 0.115 & 0.152 & 0.197 & 0.210 & 0.178 & 0.111 & 0.129 & 0.135 & 0.165 & 0.134 & 0.139 \\
                                           & PixelNeRF~\cite{PixelNeRF_yu2021pixelnerf} & 0.084 & 0.116 & 0.105 & 0.095 & 0.146 & 0.129 & 0.114 & 0.141 & 0.066 & 0.116 & 0.098 & 0.097 & 0.111 & 0.108 \\
                                           & FE-NVS~\cite{FE_NVS_guo2022fast}    & 0.061 & 0.080 & 0.076 & 0.085 & 0.103 & 0.105 & 0.091 & 0.116 & 0.048 & 0.081 & 0.071 & 0.080 & 0.094 & 0.082 \\
                                           % & FWD       & \cb{0.034} & \cb{0.055} & \cb{0.056} & \cb{0.042} & \cb{0.081} & \cb{0.079} & \cb{0.062} & \cb{0.091} & \cb{0.026} & \cb{0.054} & \cb{0.049} & \cb{0.056} & \cb{0.052} & \cb{0.055} \\
                                           & {SRT}~\cite{srt22}       & {0.050} & {0.068} & \textbf{0.058} & {0.062} & {0.085} & {0.087} & {0.082} & {0.096} & {0.045} & {0.066} & {0.055} & \textbf{0.059} & {0.079} & {0.066} \\
                                        %  \cline{2-16} 
                                        %  &\textbf{OPP-N}& {0.051} & {0.075} & {0.077} & {0.068} & {0.096} & {0.097} & {0.084} & {0.110} & {0.045} & {0.076} & {0.061} & {0.074} & {0.077} & {0.073} \\
                                        %  &\textbf{OPP-G}& \textbf{0.035} & \textbf{0.050} & \textbf{0.058} & \textbf{0.040} & \textbf{0.068} & \textbf{0.073} & \textbf{0.052} & \textbf{0.088} & \textbf{0.027} & \textbf{0.052} & \textbf{0.044} & \textbf{0.057} & \textbf{0.048} & \textbf{0.050} \\
                                         &\textbf{OPP (ours)}& 
                            \textbf{0.038} & \textbf{0.055} & \textbf{0.058} & \textbf{0.047} & \textbf{0.073} & \textbf{0.077} & \textbf{0.060} & \textbf{0.090} & \textbf{0.031} & \textbf{0.056} & \textbf{0.046} & \textbf{0.059} & \textbf{0.057} & \textbf{0.054} \\
         \hline
      \end{tabular}
  \end{adjustbox}
  %{-3mm}
  % \vspace{-4mm}
%{-6mm}
\end{table*}

==> Table/NMR_SOTA_withNG.tex <==

\begin{table*}[t]
  
  \begin{adjustbox}{width=\linewidth,center}
      \begin{tabular}{l| l c c c c c c c c c c c c c c}
        \rowcolor[gray]{.9}
        \hline
        Metrics & Methods & plane & bench & cbnt. & car & chair & disp. & lamp & spkr. & rifle & sofa & table & phone & boat & average \\
         \hline \hline
        \multirow{6}{*}{$\uparrow$ PSNR}    & SRN       & 26.62 & 22.20 & 23.42 & 24.40 & 21.85 & 19.07 & 22.17 & 21.04 & 24.95 & 23.65 & 22.45 & 20.87 & 25.86 & 23.28 \\
                                           & PixelNeRF & 29.76 & 26.35 & 27.72 & 27.58 & 23.84 & 24.22 & 28.58 & 24.44 & 30.60 & 26.94 & 25.59 & 27.13 & 29.18 & 26.80\\
                                           & FE-NVS    & 30.15 & 27.01 & 28.77 & 27.74 & 24.13 & 24.13 & 28.19 & 24.85 & 30.23 & 27.32 & 26.18 & 27.25 & 28.91 & 27.08 \\ \cline{2-16}
                                         &\textbf{OPP-N}& \underline{31.05} & \underline{28.06} & {29.24} & \underline{28.52} & \underline{25.16} & {25.31} & {28.76} & {25.44} & \underline{31.44} & \underline{28.19} & {27.21} & {27.91} & \underline{30.06} & \underline{28.00} \\
                                         &\textbf{OPP-G}& {30.83} & {27.92} & \underline{29.33} & {28.17} & {25.10} & \underline{25.35} & \textbf{29.22} & \underline{25.49} & {31.11} & {28.05} & \underline{27.29} & \underline{28.06} & {29.76} & {27.90} \\
                                         &\textbf{OPP-RVBA}& \textbf{31.27} & \textbf{28.24} & \textbf{29.49} & \textbf{28.62} & \textbf{25.32} & \textbf{25.46} & \underline{29.15} & \textbf{25.58} & \textbf{31.54} & \textbf{28.30} & \textbf{27.43} & \textbf{28.11} & \textbf{30.11} & \textbf{28.16} \\
         \hline
        \multirow{6}{*}{$\uparrow$ SSIM}    & SRN       & 0.901 & 0.837 & 0.831 & 0.897 & 0.814 & 0.744 & 0.801 & 0.779 & 0.913 & 0.851 & 0.828 & 0.811 & 0.898 & 0.849 \\
                                           & PixelNeRF & 0.947 & 0.911 & 0.910 & 0.942 & 0.858 & 0.867 & 0.913 & 0.855 & 0.968 & 0.908 & 0.898 & 0.922 & 0.939 & 0.910 \\
                                           & FE-NVS    & 0.957 & 0.930 & 0.925 & 0.948 & 0.877 & 0.871 & 0.916 & 0.869 & 0.970 & 0.920 & 0.914 & 0.926 & 0.941 & 0.920 \\
                                        \cline{2-16}
                                        &\textbf{OPP-N}& \underline{0.961} & \underline{0.937} & {0.926} & \underline{0.953} & {0.890} & \underline{0.886} & \underline{0.921} & {0.873} & {0.974} & \underline{0.926} & {0.924} & {0.929} & \underline{0.950} & {0.929} \\
                                         &\textbf{OPP-G}& {0.960} & {0.937} & \underline{0.928} & {0.951} & \underline{0.892} & \textbf{0.890} & \textbf{0.925} & \underline{0.877} & \underline{0.975} & \underline{0.926} & \underline{0.927} & \underline{0.932} & {0.949} & \underline{0.930} \\
                                         &\textbf{OPP-RVBA}& \textbf{0.962} & \textbf{0.940} & \textbf{0.931} & \textbf{0.954} & \textbf{0.894} & \textbf{0.890} & \textbf{0.925} & \textbf{0.879} & \textbf{0.976} & \textbf{0.929} & \textbf{0.928} & \textbf{0.933} & \textbf{0.951} & \textbf{0.932} \\
         \hline
        \multirow{6}{*}{$\downarrow$ LPIPS} & SRN       & 0.111 & 0.150 & 0.147 & 0.115 & 0.152 & 0.197 & 0.210 & 0.178 & 0.111 & 0.129 & 0.135 & 0.165 & 0.134 & 0.139 \\
                                           & PixelNeRF & 0.084 & 0.116 & 0.105 & 0.095 & 0.146 & 0.129 & 0.114 & 0.141 & 0.066 & 0.116 & 0.098 & 0.097 & 0.111 & 0.108 \\
                                           & FE-NVS    & 0.061 & 0.080 & 0.076 & 0.085 & 0.103 & 0.105 & 0.091 & 0.116 & 0.048 & 0.081 & 0.071 & 0.080 & 0.094 & 0.082 \\
                                         \cline{2-16} &\textbf{OPP-N}& {0.051} & {0.075} & {0.077} & {0.068} & {0.096} & {0.097} & {0.084} & {0.110} & {0.045} & {0.076} & {0.061} & {0.074} & {0.077} & {0.073} \\
                                         &\textbf{OPP-G}& \textbf{0.035} & \textbf{0.050} & \textbf{0.058} & \textbf{0.040} & \textbf{0.068} & \textbf{0.073} & \textbf{0.052} & \textbf{0.088} & \textbf{0.027} & \textbf{0.052} & \textbf{0.044} & \textbf{0.057} & \textbf{0.048} & \textbf{0.050} \\
                                         &\textbf{OPP-RBVA}& 
                            \underline{0.041} & \underline{0.058} & \underline{0.062} & \underline{0.049} & \underline{0.076} & \underline{0.080} & \underline{0.062} & \underline{0.094} & \underline{0.033} & \underline{0.059} & \underline{0.049} & \underline{0.061} & \underline{0.059} & \underline{0.057} \\
         \hline
      \end{tabular}
  \end{adjustbox}
  
  {\caption{\textbf{Comparisons with the state-of-the-art methods under category-agnostic setting.} } 
  \label{tab:category_agnostic}}
\end{table*}

==> Table/SRN_SOTA_withNG.tex <==
\begin{table}[t]
    % \tiny
    % \footnotesize
%   \centering
   
  \resizebox{\linewidth}{!}{
% \setlength{\columnwidth}{3mm}{
\begin{tabular}{l|lcccc}
\rowcolor[gray]{.9}
\hline
                                 Category          & Methods                        & $\uparrow$ PSNR                & $\uparrow$ SSIM               & $\downarrow$ LPIPS      & $\downarrow$ FID \\ \hline \hline
\multirow{7}{*}{Chairs}                    & SRN                            & 22.89                           & 0.89                           & 0.104                      &  -                 \\
                                           
                                           & CodeNeRF                       & 22.39                           & 0.87                           & 0.166                      &    -               \\
                                           & FE-NVS                         & 23.21                           & \textbf{0.92}                           & 0.077                      &    -               \\ 
                                           & PixelNeRF                      & 23.72                           & 0.91                           & 0.128          & 38.49                  \\ \cline{2-6}
                                           & \textbf{OPP-N} & {23.99}      & \textbf{0.92}     & {0.084} & 26.62                   \\
                                           & \textbf{OPP-G} & {23.57}      & \textbf{0.92}     & \textbf{0.066} & 16.95                   \\
                                           & \textbf{OPP-RVBA} & \textbf{24.05}      & \textbf{0.92}     & {0.070} &
                \textbf{15.69} \\ \hline
{\multirow{7}{*}{Cars}} & SRN                            & 22.25                           & 0.89                           & 0.129                      &    -               \\
\multicolumn{1}{c|}{}                      & CodeNeRF                       & 22.73                           & 0.89                           & 0.128                      &       -            \\
\multicolumn{1}{c|}{}                      & FE-NVS                         & 22.83                           & \textbf{0.91} & 0.099                      &            -       \\
\multicolumn{1}{c|}{}                      & PixelNeRF                      & 23.17 & 0.90                           & 0.146                      &   59.15             \\ \cline{2-6}
\multicolumn{1}{c|}{}                      & \textbf{OPP-N} & {23.21}      &  \textbf{0.91}     & {0.109} &  52.22                 \\
\multicolumn{1}{c|}{}                      & \textbf{OPP-G} & {22.72}      & {0.90}     & \textbf{0.085} &   32.14               \\
\multicolumn{1}{c|}{}                      & \textbf{OPP-RVBA} & \textbf{23.24}      &  \textbf{0.91}     & {0.092} &    \textbf{31.19}              \\ \hline
\end{tabular}
    %   }
    }
    
    \caption{\textbf{ Comparisons with the state-of-the-art methods under category-specific setting.} The performance of our final One-stage Parallel Pipeline (OPP) is reported. ``-N'' represents the NeRF paradigm of DPS which performs better at realness metrics (PSNR, SSIM), while ``-G'' indicates the generative paradigm that is better at sharpness metrics (LPIPS, FID). With the proposed RVBA, we achieve the final novel view images with both high realness and sharpness compared with previous state-of-the-art methods. }
  \label{tab:category_specific}
\end{table}

==> Table/Unsupervised_NeRF_GAN.tex <==
\begin{table}[t]
    \setlength{\abovecaptionskip}{0cm}
    \footnotesize
     \caption{\textbf{Comparisons with the unsupervised NeRF-GAN methods on the chairs category of ShapeNet under the category-specific setting.} ``*'': In line with Pix2NeRF, FID in $64\times64$ resolution is reported. }
     \label{tab:unsupervised_nerf_gan}
  % \resizebox{\linewidth}{!}{
% \setlength{\columnwidth}{15mm}{
% \vspace{-4mm}
\setlength\tabcolsep{15.5pt}
    \begin{tabular}{l|ccc}
        \rowcolor[gray]{.9}
        \hline
        Methods           & $\uparrow$ PSNR   & $\uparrow$ SSIM                               & $\downarrow$ FID*   \\ \hline \hline
        
        $\pi$-GAN~\cite{PiGAN_chan2021pi}     & - & -                                           &  15.47   \\                                
        Pix2NeRF~\cite{Pix2NeRF_cai2022pix2nerf}  & {18.14}  & 0.84                                                 &  14.31   \\
        \textbf{OPP (ours)} & \textbf{24.03}  & \textbf{0.92}      & \textbf{7.86} \\ 
        \hline
        \end{tabular}
    % }
    % \vspace{-2mm}
\end{table}

% 7.86468820826974
